Quantitative Evaluation Approach for Translation of Perceptual Soundscape Attributes: Initial Application to the Thai Language

Translation of perceptual soundscape attributes from one language to another remains a challenging task that requires a high degree of fidelity in both psychoacoustic and psycholinguistic senses across the target population. Due to the inherently subjective nature of human perception, translating soundscape attributes using only small focus group discussion or expert panels could lead to translations with psycholinguistic meanings that, in a non-expert setting, deviate or distort from that of the source language. In this work, we present a quantitative evaluation method based on the circumplex model of soundscape perception to assess the overall translation quality across a set of criteria. As an initial application domain, we demonstrated the use of the quantitative evaluation framework in the context of an English-to-Thai translation of soundscape attributes.

==> citealias.tex <==
\defcitealias{InternationalOrganizationforStandardization2014ISOFramework}{ISO, 2014} 

\defcitealias{InternationalOrganizationforStandardization2018ISO/TSRequirements}{ISO, 2018} 

\defcitealias{InternationalOrganizationforStandardization2019ISO/TSAnalysis}{ISO, 2019}

\defcitealias{InternationalOrganizationforStandardization2007ISOLanguage}{ISO, 2007}
